SonoSAMTrack -- Segment and Track Anything on Ultrasound Images

In this paper, we present SonoSAMTrack - that combines a promptable foundational model for segmenting objects of interest on ultrasound images called SonoSAM, with a state-of-the art contour tracking model to propagate segmentations on 2D+t and 3D ultrasound datasets. Fine-tuned and tested exclusively on a rich, diverse set of objects from $\approx200$k ultrasound image-mask pairs, SonoSAM demonstrates state-of-the-art performance on 7 unseen ultrasound data-sets, outperforming competing methods by a significant margin. We also extend SonoSAM to 2-D +t applications and demonstrate superior performance making it a valuable tool for generating dense annotations and segmentation of anatomical structures in clinical workflows. Further, to increase practical utility of the work, we propose a two-step process of fine-tuning followed by knowledge distillation to a smaller footprint model without comprising the performance. We present detailed qualitative and quantitative comparisons of SonoSAM with state-of-the-art methods showcasing efficacy of the method. This is followed by demonstrating the reduction in number of clicks in a dense video annotation problem of adult cardiac ultrasound chamber segmentation using SonoSAMTrack.

==> PromptSegLit.tex <==
\section{Related Prior Literature}

In this section we provide a brief overview of the prior literature related to promptable segmentation methods. The user prompts can be captured in different ways like scribbles \cite{scribbles1,scribbles2}, bounding box \cite{bbox1,bbox2}, extreme points \cite{extreme}, clicks, texts and images \cite{PhraseClick, CLIP}. Among these the clicks have been most explored due to their simplicity and intuitivenes. Bounding box and extreme points demands more effort from users in terms of capturing the extents accurately; scribbles pose difficulty in terms of simulating user behavior during training. Text and image based prompts require additional annotations in terms of text and object labels. Early click based segmentation approaches formulated the task as an optimization problem of obtaining similar, connected region with reference to the region identified by the user prompt. These early approches utilized graph based approaches \cite{GraphCut}, gaussian mixture models \cite{GrabCut}, and other related methods. Broadly these methods rely on strongly specified representation of semantic information and thus would demand large amount of user prompts to complete the task. First use of deep learning combined input image with user clicks represented as distance maps as input for a CNN to predict a segmentation mask \cite{DeepCut}. Several advancements were explored to improve the performance of learning methods \cite{BRS,fBRS}. RITM \cite{RITM} significanty improved the effectiveness of learning based approaches with the use of an iterative sampling strategy to generate clicks during training \cite{iterativeClick} and use of high quality images, annotations. FocalClick \cite{FocalClick} utilizes localized inference strategy to further improve accuracy, responsiveness and lowered compute requirements. SimpleClick \cite{SimpleClick} explored the use of vision transformers for interacitve segmentation and their potential as foundation models. SAM \cite{SAM} extended this to multiple prompts, via encodings, and trained on large scale data to enable several mainstream applications including zero-shot segmentation.

\begin{thebibliography}	

\bibitem{article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{scribbles1}
J. Bai, X. Wu, Error-tolerant scribbles based interactive image segmentation. CVPR (2014).
\bibitem{scribbles2}
T. H. Kim, K. M. Lee, S. U. Lee, Generative image segmentation using random walks with restart. ECCV (2008).
\bibitem{bbox1}
S. Zhang, J. H. Liew, Y. Wei, S. Wei, Y. Zhao, Interactive object segmentation with inside-outside guidance. (CVPR) 2020.
\bibitem{bbox2}
J. Wu, Y. Zhao, J.-Y. Zhu, S. Luo, Z. Tu, MILCut: A sweeping line multiple instance learning paradigm for interactive image segmentation. CVPR (2014).
\bibitem{extreme}
K.-K. Maninis, S. Caelles, J. Pont-Tuset, L. V. Gool, Deep extreme cut: From extreme points to object segmentation. CVPR (2018).

\bibitem{GrabCut}
C. Rother, V. Kolmogorov, A. Blake, “GrabCut”: interactive foreground extraction using iterated graph cuts, ACM Transactions on Graphics 23 (2004).
\bibitem{GraphCut}
Y. Boykov, M.-P. Jolly, Interactive graph cuts for optimal boundary & region segmentation of objects in n-d images. ICCV (2001).
\bibitem{RandomWalk}
L. Grady, Random walks for image segmentation. IEEE Trans. PAMI 28 (2006).
\bibitem{Geodesic}
V. Gulshan, C. Rother, A. Criminisi, A. Blake, A. Zisserman, Geodesic star convexity for interactive image segmentation. CVPR (2010). 

\bibitem{DeepCut}
N. Xu, B. Price, S. Cohen, J. Yang, T. Huang, Deep interactive object selection. CVPR (2016).

\bibitem{CLIP}
Alec Radford, Jong Wook Kim, Chris Hallacy, Aditya Ramesh, Gabriel Goh, Sandhini Agarwal, Girish Sastry, Amanda Askell, Pamela Mishkin, Jack Clark, et al. Learning transferable visual models from natural language supervision. ICML (2021).

\bibitem{RITM}
Konstantin Sofiiuk, Ilia A Petrov, and Anton Konushin. Reviving iterative training with mask guidance for interactive segmentation. arXiv:2102.06583 (2021).

\biitem{iterativeClick}
S. Mahadevan, P. Voigtlaender, B. Leibe, Iteratively trained interactive segmentation. BMVC (2018).

\bibitem{99percent}
Marco Forte, Brian Price, Scott Cohen, Ning Xu, and Franc¸ois Piti´e. Getting to 99% accuracy in interactive segmentation. arXiv:2003.07932 (2020).

\bibitem{BRS}
Won-Dong Jang and Chang-Su Kim. Interactive image segmentation via backpropagating refinement scheme. In CVPR, 2019.

\bibitem{fBRS}
Konstantin Sofiiuk, Ilia Petrov, Olga Barinova, and Anton Konushin. f-brs: Rethinking backpropagating refinement for interactive segmentation. CVPR (2020).

\bibitem{FocalClick}
Xi Chen, Zhiyan Zhao, Yilei Zhang, Manni Duan, Donglian Qi, and Hengshuang Zhao. FocalClick: towards practical interactive image segmentation. CVPR (2022).

\bibitem{SimpleClick}
Qin Liu, Zhenlin Xu, Gedas Bertasius, and Marc Niethammer. SimpleClick: Interactive image segmentation with simple vision transformers. arXiv:2210.11006 (2022).

\bibitem{SAM}
Kirillov, A., Mintun, E., Ravi, N., Mao, H., Rolland, C., Gustafson, L., and Girshick, R. (2023). Segment anything. arXiv preprint arXiv:2304.02643

\bibitem{PhraseClick}
. Ding, S. Cohen, B. Price, X. Jiang, PhraseClick: Toward achieving flexible interactive segmentation by phrase and click. ECCV (2020)

\end{thebibliography}
\end{document}

